Boosting the Performance of Decentralized Federated Learning via Catalyst Acceleration

Decentralized Federated Learning has emerged as an alternative to centralized architectures due to its faster training, privacy preservation, and reduced communication overhead. In decentralized communication, the server aggregation phase in Centralized Federated Learning shifts to the client side, which means that clients connect with each other in a peer-to-peer manner. However, compared to the centralized mode, data heterogeneity in Decentralized Federated Learning will cause larger variances between aggregated models, which leads to slow convergence in training and poor generalization performance in tests. To address these issues, we introduce Catalyst Acceleration and propose an acceleration Decentralized Federated Learning algorithm called DFedCata. It consists of two main components: the Moreau envelope function, which primarily addresses parameter inconsistencies among clients caused by data heterogeneity, and Nesterov's extrapolation step, which accelerates the aggregation phase. Theoretically, we prove the optimization error bound and generalization error bound of the algorithm, providing a further understanding of the nature of the algorithm and the theoretical perspectives on the hyperparameter choice. Empirically, we demonstrate the advantages of the proposed algorithm in both convergence speed and generalization performance on CIFAR10/100 with various non-iid data distributions. Furthermore, we also experimentally verify the theoretical properties of DFedCata.

==> tex/bio.tex <==

\vspace{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/qinglunli.png}}]{Qinglun Li}
obtained his bachelor’s degree in Science from the School of Science at the University of Shanghai for Science and Technology. He is pursuing a doctorate in Management Science and Engineering at the National University of Defense Technology. His research interests include machine learning, decentralized federated learning, and non-convex optimization. He has served as ICML 2024 and ICLR 2025 reviewer.
% \vspace{-1cm}
\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{bio/zhangmiao.jpg}}]{Miao Zhang} is currently a research assistant at National University of Defense Technology, Changsha, China. He received his bachelor’s degree from the School of Information, University of Science and Technology of China in 2015, and received his master’s degree and Ph.D. from the College of Systems Engineering, National University of Defense Technology in 2017 and 2022, respectively. His research interests include intelligence optimization, resource management, private computing, federated learning and reinforcement learning.
\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yingqi.png}}]{Yingqi Liu}
% or if you just want to reserve a space for a photo:
received the B.Sc. degree and  M.Sc. degree in Electronic and Information Science from the School of Electronic and Optical Engineering, Nanjing University of Science and Technology, Nanjing, China,
in 2021 and 2024. Her research interests include computer vision, federated learning, and distributed optimization.
\end{IEEEbiography}
\vspace{-1cm}





\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{bio/quanjun.pdf}}]{Quanjun yin} is currently a professor with the College of Systems Engineering, National University of Defense Technology, China. His research interests include cognitive process modelling, qualitative spatial reasoning and planning, cooperation and negotiation, cloud-based simulation, and edge computing.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/li_shen.png}}]{Li Shen} is currently an associate professor at Sun Yat-sen University. Previously, he was a research scientist at JD Explore Academy, Beijing, and a senior researcher at Tencent AI Lab, Shenzhen. He received his bachelor's degree and Ph.D. from the School of Mathematics, South China University of Technology. His research interests include theory and algorithms for nonsmooth convex and nonconvex optimization, and their applications in trustworthy artificial intelligence, deep learning, and reinforcement learning. He has published more than 100 papers in peer-reviewed top-tier journal papers (JMLR, IEEE TPAMI, IJCV, IEEE TSP, IEEE TIP, IEEE TKDE, etc.) and conference papers (ICML, NeurIPS, ICLR, CVPR, ICCV, etc.). He has also served as the senior program committee for AAAI 2022, and AAAI 2024 and area chairs for ICML 2024, ICLR 2024, ICPR 2022, and ICPR 2024.
% \vspace{-1cm}
\end{IEEEbiography}
\vspace{-1cm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/xiaochuncao.jpg}}]{Xiaochun Cao}
	(Senior Member, IEEE) received the B.E. and M.E. degrees in Computer Science from Beihang University, Beijing, China, in 1999 and 2002, respectively, and the Ph.D. degree in Computer Science from the University of Central Florida, Orlando, FL, USA, in 2006. After graduation, he spent about three years at ObjectVideo Inc., as a Research Scientist. From 2008 to 2012, he was a Professor at Tianjin University, Tianjin, China. Before joining Sun Yat-sen University, Shenzhen, China, he was a Professor at the Institute of Information Engineering, Chinese Academy of Sciences, Beijing, China. He is a Professor and the Dean with the School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen University. He has published more than 200 journal and conference papers. Dr. Cao’s dissertation was nominated for the University Level Outstanding Dissertation Award. He was a recipient of the Piero Zamperoni Best Student Paper Award at the \emph{International Conference on Pattern Recognition}, in 2004 and 2010. He was on the Editorial Boards of \emph{IEEE Transactions on Circuits and Systems for Video Technology} and \emph{IEEE Transactions on Multimedia}. He is on the Editorial Boards of \emph{IEEE Transactions on Pattern Analysis and Machine Intelligence} and \emph{IEEE Transactions on Image Processing}.
\end{IEEEbiography}


